Theory and Experiments on Vector Quantized Autoencoders

Deep neural networks with discrete latent variables offer the promise of better symbolic reasoning, and learning abstractions that are more useful to new tasks. There has been a surge in interest in discrete latent variable models, however, despite several recent improvements, the training of discrete latent variable models has remained challenging and their performance has mostly failed to match their continuous counterparts. Recent work on vector quantized autoencoders (VQ-VAE) has made substantial progress in this direction, with its perplexity almost matching that of a VAE on datasets such as CIFAR-10. In this work, we investigate an alternate training technique for VQ-VAE, inspired by its connection to the Expectation Maximization (EM) algorithm. Training the discrete bottleneck with EM helps us achieve better image generation results on CIFAR-10, and together with knowledge distillation, allows us to develop a non-autoregressive machine translation model whose accuracy almost matches a strong greedy autoregressive baseline Transformer, while being 3.3 times faster at inference.

==> experiments.tex <==
We  trained the unconditional discrete latent model on CIFAR-10, achieving very similar negative log perplexity as \citep{vqvae}. We measure
We maintain the same encoder and decoder architecture as MT. Our latent prediciton model, uses an image transformer\citep{imagetrans} autoregressive decoder with local $1D$ attention. We generate 8x8x10 discrete latents, same as \citep{vqvae}, with a codebook size of $256$, each containing $512$ dimensions. We use $4$ convolutional layers followed by 2 residual layers and a single $1x1$ conv layer. 

==> model.tex <==
Our models and generative process follow \cite{vqvae} for unconditional image generation, and \cite{kaiser2018fast} for neural machine translation. Note that for unconditional image generation, we model the joint probability $P(x, z)$ where $x$ is the image, and model $P(y, z \mid x)$ for machine translation, where $y$ and $x$ are the target and source sentence respectively. The models have two basic components:

\paragraph{AutoEncoder.} The autoencoder comprises an encoder function $\cae$, that compresses the output, which is $x$ in image generation and $y$ in neural machine translation, to a continuous representation followed by a bottleneck function that discretizes the output of the encoder, and finally a decoder function, that generates $x$ or $y$. For both unconditional image generation and machine translation, the encoder is a series of strided convolutional layers with residual convolutional layers in between. In machine translation, the encoder of the autoencoder \marginpar{this should all be replaced with variables} can optionally attend to the continuous representation of the input, $x$ in this case, which is computed with the self-attention based encoder from the Transformer model. We use DVQ and Semhash for the discretization algorithm. The decoders, applied after the bottleneck layer, differ for the two tasks: we use successive layers of transposed convolutions image generation that generate the image, and for machine translation, we also use transposed convolution layers whose continuous output is fed to a transformer decoder with causal attention, which generates the output.

\paragraph{Language Model.} In both tasks, we use a Transformer decoder to model $P(z)$ and $P(z|x)$, using multi-head encoder-decoder attention to model the conditioning on $x$ in machine translation.
